Complex Organics Surrounding the FU Ori-Type Object V1057 Cyg Indicative of Sublimated Ices

FU Ori and EX Lup type objects present natural experiments for understanding a critical stage in the star and planet formation process. These objects offer insight into the diversity of molecules available to forming planetary systems due to a sudden increase in accretion and central luminosity causes the disk and surrounding material to increase in temperature. This allows for volatiles to sublimate off of grains and exist in the gas-phase for tens to hundreds of years post initial outburst. While this dynamic stage may be common for solar-type protostars, observations of the chemical impact of these bursts are rare. In this article, we present observations from the NOrthern Extended Millimeter Array (NOEMA) of five Young Stellar Objects (YSOs) that have undergone outbursts within the past 100 years and catalog the volatile chemistry found within approx 1000 au of the YSO. Only one source clearly shows a line rich spectra with >11 molecules detected including complex organics and water, as is an expected spectra signature for a post-outburst source. This source is V1057 Cyg, and we present it as the northern analog to the well studied and molecule-rich FU Ori source, V883 Ori. Our conclusions on the chemical inventory of the other four sources in our sample are sensitivity limited, as V1057 Cyg contains the highest disk/envelope gas mass.

==> molecular_tables.tex <==
\begin{deluxetable*}{cccccccc}
\label{tab:Common lines}
\tablecolumns{7}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{Identified Lines Across all Outburst Sources}
\tablehead{Molecule	&	Transition	&	Frequency (GHz)	& V1057 Cyg &	V1515 Cyg	&	V1647 Ori	&	V1735 Cyg	&	V2492 Cyg}
\startdata
\ce{^{13}CO}	&	J=2-1	&	220.399	& yes &	yes	&	yes	&	yes	&	yes	\\
\ce{C^{18}O}	&	J=2-1	&	219.560	& yes&	yes	&	yes	&	yes	&	yes	\\
\ce{C^{17}O}	&	J=2-1	&	224.714	& yes&	yes	&	yes	&	yes	&	yes	\\
SO	&	4(5)- 3(4)	&	206.176	& yes&	yes	&	yes	&	yes	&	yes	\\
SO	&	6(5)-5(4)	&	219.949	& yes&	yes	&	yes	&	yes	&	yes	\\
\ce{SO2}	&	12(0,12)-11(1,11)	&	203.392	& yes &	maybe	&		&		&		\\
\ce{SO2}	&	11(2,10)- 11(1,11)	 &	205.301	& yes  &		&		&	maybe	&		\\
\ce{H2CO}	&	3(0,3)-2(0,2)	& 	218.222	& yes &	yes	&	yes	&	yes	&	yes	\\
\ce{H2CO}	&	3(1,2)-2(1,1)	&	225.698	& yes &	yes	&	yes	&	yes	&	yes	\\
\ce{H2CO}	&	3(2,2)-2(2,1)	&	218.476	& yes &		&		&	maybe	&	yes	\\
\ce{H2CO}	&	3(2,1)-2(2,0)	&	218.760	& yes &		&		&	yes	&	maybe	\\
\enddata
\tablecomments{All of the above molecules and transitions have a bright detection in source V1057 Cyg, and either have a bright detection (noted with `yes') or tentative detection (noted with `maybe') in each corresponding source. }
\end{deluxetable*}

\colorlet{color1}{green!10!white}
\colorlet{color2}{cyan!10!white}
\colorlet{color3}{red!10!white}
\colorlet{color4}{olive!10!white}

\begin{deluxetable*}{ccc}
\label{tab:Bonus_lines}
\tablecolumns{3}
\tablewidth{0pt}
\tabletypesize{\small}
\tablecaption{Additional Identified Lines In V1057 Cyg}
\tablehead{Molecule	&	Transition	&	Frequency (GHz)}
\startdata
\rowcolor{color1} \multicolumn{3}{c}{Carbon Isotopologue}\\
\ce{^{13}C^{18}O}	&	2-1	&	209.419	\\
\rowcolor{color2} \multicolumn{3}{c}{Water}\\			
HDO	&	3( 1, 2)- 2( 2, 1)	&	225.897	\\	
\rowcolor{color3} \multicolumn{3}{c}{Sulfur Species}\\
OCS	&	17-16	&	206.745	\\
OCS	&	18-17	&	218.903	\\
\ce{SO2}	&	3( 2, 2)- 2( 1, 1)	&	208.700	\\
\ce{SO2}	&	11( 1,11)-10( 0,10)	&	221.965	\\
\ce{SO2}	&	20( 2,18)-19( 3,17)	&	224.265	\\
\ce{SO2}	&	13( 2,12)-13( 1,13)	&	225.154	\\
\ce{H2CS}	&	6( 1, 6)- 5( 1, 5)	&	202.924	\\
\ce{H2CS}	&	6( 0, 6)- 5( 0, 5)	&	205.988	\\
\ce{H2CS}	&	6( 1, 5)- 5( 1, 4)	&	209.200	\\
\rowcolor{color4} \multicolumn{3}{c}{Building-block COMs}\\		
\ce{CH3CN }	&	12-11 k = 3	&	220.709	\\
\ce{CH3CN} 	&	12-11 k = 2	&	220.730	\\
\ce{CH3CN} 	&	12-11 k = 1	&	220.743	\\
\ce{CH3CN} 	&	12-11 k = 0	&	220.747	\\
\ce{H3CN}	&	23-22	&	209.230	\\
\ce{H3CN}	&	24-23	&	218.325	\\
\ce{H2^{13}CO}	&	3( 1, 3)- 2( 1, 2)	&	206.132	\\
\ce{H2^{13}CO}	&	3(1,2)-2(1,1)	&	219.908	\\
\ce{CH3OH}	&	1( 1) + - 2( 0) + vt=0	&	205.791	\\
\ce{CH3OH}	&	4(2,2)-3(1,2)	&	218.440	\\
\ce{CH2DOH}	&	10(1,9) - 9(1,8)	&	203.937	\\
\ce{CH2DOH}	&	7(2,6) - 7(1,7), e1	&	224.701	\\
\rowcolor{LightYellow} \multicolumn{3}{c}{Long COMs}\\			
\ce{CH3OCH3}	&	11( 1,11)-10( 0,10)	&	209.515	\\
\ce{CH3OCHO}	&	18( 6,13)- 17( 6,12) E	&	224.022	\\
\ce{CH3OCHO}	&	8( 5,14)- 17( 5,13) A	&	224.328	\\
\enddata
\tablecomments{These molecules and associated transitions show up as bright detections. There are more long COMs with tentative detections that will be used to confirm the existence of these COMs in V1057 Cyg}
\end{deluxetable*}

\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{images/Line_rich_example.pdf}
    \caption{\textit{An example of the spectra of the central pixel of each source between 218.2-219 GHz. This region shows how V1057 Cyg is markedly more line-rich than each of the other sources. }}
    \label{fig:line-rich-example}
\end{figure*}
